A Latent Space Analysis of Editor Lifecycles in Wikipedia

Collaborations such as Wikipedia are a key part of the value of the modern Internet. At the same time there is concern that these collaborations are threatened by high levels of member turnover. In this paper we borrow ideas from topic analysis to editor activity on Wikipedia over time into a latent space that offers an insight into the evolving patterns of editor behavior. This latent space representation reveals a number of different categories of editor (e.g. content experts, social networkers) and we show that it does provide a signal that predicts an editor's departure from the community. We also show that long term editors gradually diversify their participation by shifting edit preference from one or two namespaces to multiple namespaces and experience relatively soft evolution in their editor profiles, while short term editors generally distribute their contribution randomly among the namespaces and experience considerably fluctuated evolution in their editor profiles.

==> conclusion.tex <==
%!TEX root = WikiProject_Membership_Turnover.tex
\section{Conclusion}
We have empirically examined the impact of membership turnover in online groups on its productivity. The results show that membership turnover has significant negative effect on group outcomes in Wikipedia, and that social capital losses through member turnover are associated with group productivity in a negative curvilinear fashion. Our results show that the loss of social capital in collaboration networks can explain significant amount of variation in productivity for WikiProjects. The results contribute to the existing literature that investigates the relationship between social capital losses and group performance (e.g., \cite{Huselid1995,Abelson1984,Shaw2005,Ransbotham2011}) in conventional organizations and online communities. The results also support the mediation of turnover rate and network density on the relationship between social capital losses and group productivity.

Previous studies have suggested that editors with different tenure are likely to perform different types of tasks \citep{Bryant2005}, and that groups consisting of members with diversified tenure generally enjoy better task distribution and group performance \citep{Chen2010}. Similarly, our exploration of the dataset reveals that projects with low levels of social capital losses and turnover rate generally enjoy better task distribution and group outcomes. It will be very interesting to investigate the impact of task distribution among members on group performance and to study the evolution of user behaviors in online communities. Furthermore, we observe that project members denote substantial amount of time to edit non main namespaces such as article talk pages and user talk pages. This study only considers social capital losses in collaboration networks, it will be worthwhile to take into account social capital losses in communication networks for WikiProjects and in article talk networks and user talk networks.


==> discussion.tex <==
%!TEX root = WikiProject_Membership_Turnover.tex
\section{Discussion}
We have found that there is a negative curvilinear relationship between social capital losses and group productivity in WikiProjects -- as social capital losses increases from very low level to moderate level, the amount of work done by project members declines; after the moderate level, with any further increased in social capital losses from turnover, the amount of work done by project members increases.

\begin{figure}[!htb]
\baselineskip=12pt
{\fontsize{10.0pt}{10.0pt}\selectfont
\begin{center}
  \subfloat{\includegraphics[width=0.90\textwidth]{./figs/Edit_Distribution_for_WP_Medicine}}\quad
  \subfloat{\includegraphics[width=0.90\textwidth]{./figs/Edit_Distribution_for_WP_Unionism_In_Ireland}}\\
\caption{Evolution of Edit Distribution for WP Medicine and WP Unionism in Ireland.}
\label{fig:Edit_Distribution_Exploration}
\end{center}
}
\end{figure}
To further understand the characteristics of quarterly observations that locate at different areas (specifically, the far left, middle and top right area) of the curve in Figure \ref{fig:sc_losses_productivity}, we explore the dataset in more details by tracking the evolution of independent variables and average task distribution over quarters. Following other studies, we also quantify different types of tasks as edits to different types of pages within Wikipedia. The file system of Wikipedia is subdivided into ``namespaces"\footnote{http://en.wikipedia.org/wiki/Wikipedia:Namespace} which represent general categories of pages based on their function. Average task distribution is calculated as the average number of edits to a specific namespace by project members in a quarter. We observe that healthy WikiProjects generally experience lower levels of member turnover and social capital losses, thus enjoy better group outcomes and better task distribution, and tend to locate somewhere between the far left and middle areas of the curve in Figure \ref{fig:sc_losses_productivity}; while unhealthy WikiProjects generally experience more fluctuation in member turnover and social capital losses, have extremely unbalanced task distribution, and have their quarterly observations distributed over the three areas of the curve in Figure \ref{fig:sc_losses_productivity}.
\begin{figure}[!htb]
\baselineskip=12pt
{\fontsize{10.0pt}{10.0pt}\selectfont
\begin{center}
  \subfloat{\includegraphics[width=0.90\textwidth]{./figs/Evolution_of_Independent_Variables_for_WP_Medicine}}\quad
  \subfloat{\includegraphics[width=0.90\textwidth]{./figs/Evolution_of_Independent_Variables_for_WP_Unionism_In_Ireland}}\\
\caption{Evolution of Independent Variables for WP Medicine and WP Unionism in Ireland.}
\label{fig:Independent_Variable_Exploration}
\end{center}
}
\end{figure}

We found that WikiProject Medicine is a very healthy project with all its observations located at the far left region of the curve, while WikiProject Unionism in Ireland is a less healthy project. Figure \ref{fig:Edit_Distribution_Exploration} and Figure \ref{fig:Independent_Variable_Exploration} present the evolution of edit distribution and independent variables for the two projects, respectively. Because article edits generally account for more that 50\% of members' activity, we omitted it from Figure \ref{fig:Edit_Distribution_Exploration} to improve readability of the graph. The two figures in Figure \ref{fig:Edit_Distribution_Exploration} shows a substantial difference among their average edit distribution: WikiProject Medicine enjoys better and more balanced task distribution than WikiProject Unionism in Ireland, with the members of the former making edits across a range of namespaces each quarter. The figures in Figure \ref{fig:Independent_Variable_Exploration} reveals that WikiProject Unionism in Ireland experiences substantial fluctuation in its member turnover and social capital losses, while WikiProject Medicine has a more stable evolution in its independent variables.
